Neural Attention for Image Captioning: Review of Outstanding Methods

Image captioning is the task of automatically generating sentences that describe an input image in the best way possible. The most successful techniques for automatically generating image captions have recently used attentive deep learning models. There are variations in the way deep learning models with attention are designed. In this survey, we provide a review of literature related to attentive deep learning models for image captioning. Instead of offering a comprehensive review of all prior work on deep image captioning models, we explain various types of attention mechanisms used for the task of image captioning in deep learning models. The most successful deep learning models used for image captioning follow the encoder-decoder architecture, although there are differences in the way these models employ attention mechanisms. Via analysis on performance results from different attentive deep models for image captioning, we aim at finding the most successful types of attention mechanisms in deep models for image captioning. Soft attention, bottom-up attention, and multi-head attention are the types of attention mechanism widely used in state-of-the-art attentive deep learning models for image captioning. At the current time, the best results are achieved from variants of multi-head attention with bottom-up attention.

==> sec3_old.tex <==

\section{Background}\label{sec3}

\subsection{Word Embeddings}
%\par
%Processing textual information is an important step in image captioning. A dataset suited for
%image captioning contains images and sentence pairs for the images. The COCO \cite{MS_COCO} dataset
%provides us with five captions for each input image. This enables measuring suitability and saliency of
%the object references in the captions and fluency of the generated caption by learning the common sense between
%a set of ground truth captions written by human annotators.
%\par
%Preprocessing the textual information for image captioning also involves creating a dictionary from the captions using n-gram calculations.
%N-grams are frequency counts and are calculated based on the number of occurrences of words in a corpus.
%After the frequencies of the words are computed, we could get rid of the least frequent words by
%inserting the ``unknown'' token for these words in the caption sentences.
%This is usually done by considering a frequency threshold of five. To be specific, words that are
%used less than five times are considered unknown words that are replaced with the ``unknown'' token.
\par
The word embeddings are vector representations of the tokens that are fed to a deep learning model. This creates the ability to learn
patterns for the words in a sentence in a shared embedded space.
The use of word embeddings enables a neural network to easily perform computations with words.
The most common embedding systems used for natural language processing
tasks are Glove \cite{Glove} and Word2vec \cite{Word2vec}.
\par 
After text preprocessing, we use the dictionary and the corpus of captions to
create embeddings for each word in the caption sentence for input to the neural model.
This mechanism of training simultaneously with image features and word embeddings allows the deep learning models to learn
the relationships between the words in the caption sentence for the input
image and the visual features of the same image in an embedded visual space.
Recurrent neural networks such as
long short-term memory networks (LSTMs) \cite{LSTM} and gated recurrent units (GRUs) \cite{GRU}
are used to map embedded words to visual features in an embedded visual space.
\par
%%########################################%########################################%########################################
%
%%########################################%########################################%########################################
%\subsection{Image Processing}
%Convolutional neural networks (CNNs) were originally designed and used for image classification \cite{CNNLecunNet1,Lecun_Bengio,CNNOriginal}.
%After training a CNN on image classification task on a huge dataset such as the ImageNet \cite{imagenet_cvpr09},
%we remove the last softmax feed-forward layer that is used for image classification from
%the CNN model. This mechanism provides us with a CNN backbone that includes convolutional layers that could be used for feature extraction from unseen images. 
%The CNN backbone that is used for feature extraction among majority of attentive deep learning models for image captioning is ResNet101 \cite{Resnet}.
%\par

%########################################%########################################%########################################

%########################################%########################################%########################################
\subsection{Generating \& Evaluating Captions}\label{sec5.2}
%\par
%In this survey, we have discussed how attention mechanisms are used to form attentive encoder-decoder models for image captioning. Now, we
%focus on the way models generate captions and how we evaluate the quality of captions generated by the models. 
\par
After training the attentive model, at test time we use the attentive model for decoding word embedding at time step $t$ regarding the
region $i$ given at time step $t$. The length of the sequence is adaptively learned by the model but usually a maximum length of sixteen words for each
caption is applied. These constraints are usually discovered based on the average length of captions in the caption dataset.
\par
In order to understand the quality of generated captions,
automatic metrics have been used widely.
Without the need for manually verifying the quality of captions by a human agent,
automatic metrics such as BLEU\cite{BLEU_2002}, METEOR\cite{METEOR}, ROUGE\cite{ROUGE}, CIDER\cite{CIDER} and SPICE\cite{SPICE}
provide excellent insight regarding the quality
of captions, from different viewpoints.
\par
Originally designed for translation tasks and focusing on the textual aspect of input information,
BLEU\cite{BLEU_2002}, METEOR\cite{METEOR} and ROUGE\cite{ROUGE},
provide numeric evaluation of the quality of translation from the input sequence to the output sequence based on n-gram calculations.
Visual information is not considered when creating scores for these metrics and only the textual information regarding the input sequence 
and output sequence is considered.
\par
In order to overcome the issue of not being able to consider visual
information for generating automatic metric scores,
Vedatanam et al. \cite{CIDER} introduced the CIDER score.
By employing term frequency and invert document frequency (TF-IDF),
this metric evaluates the quality of a set of candidate sentences with
a set of reference sentences, given an input image. For the first time,
this metric provided researchers with a way to evaluate
the quality of generated captions considering the fluency and relevancy,
fluency in caption sentence, and the relevancy between 
the caption sentence and input image. 
\par
Although the CIDER\cite{CIDER} metric was successful in assessing
relevancy between the images and sentences, there was no way to
verify the existence or truth regarding the presence of spatial relationships among the objects in the given image,
as described in the caption sentence generated by a model.
For this purpose, Anderson et al. introduced the SPICE\cite{SPICE} metric, 
which employs scene graphs in order to verify the spatial
relationships among the objects, described in the caption.
The survey by Liu et al. \cite{Liu2019_survey} offers useful details and information regarding how the evaluation metrics are designed. Therefore we
avoid reiterating the same information here.
\par

==> sec4_old.tex <==

\section{Attentive Deep Learning for Image Captioning}\label{sec4}
\par
We categorize the papers reviewed for our survey, first based on the type of attention mechanisms,
second based on the nature of language models, and third based on the type of encoder.
We refer to the deep learning models that use attention mechanisms as attentive deep learning models.
In this section, we review the state-of-the-art literature
in this category. The categorization for the papers we reviewed
in this survey is illustrated in Fig. \ref{fig2}.
\par
\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth, frame={\fboxrule} {-\fboxrule}]{fig2.pdf}
    \caption{The taxonomy graph of attentive deep learning models used for image caption generation in our survey.}
    \label{fig2}
\end{figure}
\par
\subsection{Attention Mechanisms}\label{sec4.1}
\par
We have witnessed the emergence and widespread use of attention
mechanisms in deep learning models during the past few years.
Attention mechanisms have a long history in neuroscience, dating back a few decades \cite{DEUBEL1996}. 
A few years ago, attention mechanisms started to show their usefulness in deep learning models in the
context of neural machine translation \cite{ORG_Attention}. This created curiosity among researchers to investigate
the usefulness of attention mechanisms in image captioning \cite{Xu,Cho}. 
\par
There are two common types of attention mechanisms in deep learning models, soft attention \cite{ORG_Attention} and multi-head attention \cite{NIPS2017_7181}.
Other attention mechanisms are either variants or successors of soft attention or multi-head attention.
Multi-head attention uses self-attention as a building block. 
In other words, multi head attention is just a concatenation of attention heads that each contain self-attention.
Most recently published literature related to image captioning using attentive deep learning models
have used the Transformer model that includes multi-head attention. Therefore, we
categorize self-attention under multi-head attention.
%because of the fact that recently Transformers are used for image caption generation. 
\par
%-------------------------------------------------------------------------------------------------------------------------------------------------------------------
\subsubsection{Soft Attention}\label{sec4.1.1}
\par
For the task of neural machine translation, the attention mechanism designed by Bahdanau et al. \cite{ORG_Attention}, 
applied a softmax activation on linear transformation of a set of weights multiplied
by the vector that contains the information we want the model to attend over. This usually involves performing
calculation over the hidden (hypothesis) or context (memory) vector of the recurrent neural network.
A softmax activation function ensures that probabilities for all attention entities in the vector add up to one.
This enables the model to pick the most important entities in the vectors.
Usually attention values are calculated and then applied to some information by performing
element-wise multiplication between the attention values and the information we want the model to attend over.
The attention mechanism introduced by Bahdanau et al. \cite{ORG_Attention}, also known as soft attention,
lays the foundation for the employment of attention mechanisms in deep learning models.
\par
%-------------------------------------------------------------------------------------------------------------------------------------------------------------------
\subsubsection{Multi-Head Attention}\label{sec4.1.2}
\par
After attention mechanisms showed their usefulness in deep neural networks,
it became clear that advancing attention mechanisms
and employing them in better ways could lead to additional performance gains in a variety of tasks.
As we stated earlier, multi-head attention
uses self-attention as building blocks \cite{NIPS2017_7181}.
Self-attention is an attention mechanism that relates different parts
of a sequence to create a representation for that sequence \cite{NIPS2017_7181}.
The self-attention block could be considered as a function for mapping the relevance of queries and keys using a
softmax activation and element-wise multiplication, applied to the values using another element-wise multiplication \cite{NIPS2017_7181}.
Self-attention mechanisms have been used in tasks such as reading
comprehension \cite{Cheng_2016_self_att1} and text summarization \cite{Parikh_2016_self_att2}.
\par
Transformers use self-attention and multi-head attention as building blocks
and they fully rely on attention mechanisms for handling long-range and short-range dependencies in the input data.
In the past, convolutional neural networks (CNNs)
have been used for managing long-range dependencies and recurrent neural networks (RNNs) such as LSTMs or
GRUs or other simpler types of RNNs for managing short-range dependencies.
On the other hand, Transformers use self-attention and multi-head attention for
managing both long-range and short-range dependencies in the data.
\par
%-------------------------------------------------------------------------------------------------------------------------------------------------------------------
\subsection{Language Models}\label{sec4.2}
\par
The task of machine translation usually involves a language model. Language modeling is the task of mathematically mapping the words
to their associating probabilities based on their frequencies of occurrences in a given corpus of text.
Having a language model, we could map input information such as
a sequence of tokens in a query to another sequence of tokens as the answer to the query.
Usually, the language model in a deep learning model used for image captioning
acts as the decoder part of the model.
\par
\subsubsection{LSTMs}\label{sec4.2.1}
\par
Recurrent neural networks such as LSTMs and GRUs have been shown to be useful for language modeling.
The mapping needed for language modeling could be learned in a shared embedded space \cite{Word2vec} inside LSTMs or GRUs. Therefore,
LSTMs could be used for language modeling and could be considered trainable language models for image captioning.
In attentive deep learning models employing LSTMs
used for image captioning, this is usually done by concatenating
the visual features as the output of the encoder part of the model
with an embedding of a given token in the caption sentence.
This creates the input for the LSTMs used for language modeling.
\par
\subsubsection{Transformers}\label{sec4.2.2}
\par
As we stated earlier, Transformers have recently been used for image captioning as well as LSTMs and GRUs.
This is because Transformers also could be used as language models as
showed by Vaswani et al. \cite{NIPS2017_7181},
%This was further shown recently in a work by Devlin et al. \cite{BERT}, namely
%bidirectional encoder representations from transformers (BERT) that has created
%a lot of excitement recently for research related to natural language processing
%tasks such as general language understanding using GLUE \cite{Wang_GLUE_2018} benchmark and
%question answering using stanford question answering data-set (SQUAD) \cite{Rajpurkar_2016_Squad}.
naturally
making them useful in image captioning.
Deep learning models used for image captioning follow the encoder-decoder
architecture, and therefore it makes sense to improve the encoder part of Transformers
by adding a visual feature extractor.
The decoder of part of Transformers are then used for generating tokens at word level.
\par
%-------------------------------------------------------------------------------------------------------------------------------------------------------------------
\subsection{Encoders}\label{sec4.3}
\par
%The Transformer model follows the encoder-decoder architecture.
%This model includes stacks of encoder-decoder modules.
%Also the attentive deep learning models used for image captioning that employ LSTMs for generating captions
%follow the encoder-decoder architecture as well.
The encoder-decoder architecture is very useful when dealing with sequence to sequence
tasks such as neural machine translation \cite{Sutskever_2014}.
No matter what kind of decoder is used for the attentive deep captioning models,
two kinds of encoders are mainly used for extracting the visual features by the decoder
part of the models, encoders that include only CNNs or encoders that
include both CNNs and object detectors to extract the visual features.
In this section we discuss different types of encoders used in deep attentive models for image captioning.
\par
\subsubsection{CNN Encoders}\label{sec4.3.1}
\par
CNNs have shown their effectiveness in visual feature extraction in the image classification task \cite{AlexNet,VGG,Resnet}.
%This is because of the nature of the data.
The pixels in an image have longe range
dependencies between each other to form a particular pattern, and therefore CNNs are useful in
visual feature extraction for image captioning \cite{Vinyals_2015_CVPR,Donahue_2015_CVPR}.
\par
In deep neural networks for image captioning, the common softmax feed-forward classification layer is removed from the CNN,
the remainder layers could be used as a CNN backbone for extracting visual features
that could be used in higher levels of deep neural network such as LSTMs.
\par
\subsubsection{Bottom-up Encoders}\label{sec4.3.2}
\par
Object detectors have also been used as encoders alongside CNNs for image captioning.
Usually, the object detector used for image captioning
is Faster-RCNN \cite{FasterRCNN} and the most commonly used CNN backbone is ResNet101 \cite{Resnet}.
The object detector detects the region proposals, which are used to create separate
regions for feature extraction by a CNN backbone, ``This mechanism serves as bottom up attention'' \cite{Anderson2017up-down}.
Adding an object detector for the encoder part causes the model to attend over salient
regions in the image by selecting the regions with highest detection scores.
Usually, a set of region proposals are sent to a decoder module that also receives the convolutional
features for those regions using a CNN backbone.
%The most commonly used CNN backbone
%used for visual feature extraction is Res-Net101 \cite{Resnet}.  
\par
%The bottom-up attention mechanism creates the bottom-up features. Instead of using a CNN
%for extracting the features of the image as a whole,
%we use an object detector first, that will provide us with coordinates
%of bounding boxes surrounding each object in the image.
%After the coordinates of bounding boxes are discovered, these coordinates
%are used to create a separate region to become processed for feature extraction by a CNN backbone.
%Thus, bottom-up attention exists when we use an object detector in
%order to detect the regions of interest in the image for feature 
%extraction instead of using the image as a whole for feature extraction.
%For feature extraction, we need a CNN backbone again.
\subsubsection{GCN \& Bottom-up Encoders}
\par
Graph convolutional networks have also been used alongside bottom-up attention. 
Inspired by how the SPICE \cite{SPICE} metric is calculated based on a scene graph generated from the input image, graph convolutional networks (GCNs) have been
used to extract information from scene graphs by reconstructing the input graph adaptively.
Scene graphs are usually used for extracting or refining spatial relationships \cite{SPICE,Li_Jiang_2019_ieee,Yao_2018_ECCV,Wang_2019_role}.
In Section \ref{sec5.1.3}, we briefly explain the
methods reviewed in our survey that employ GCNs alongside bottom-up attention to form the encoder.
\par
%########################################%########################################%########################################

